In Pursuit of Interpretable, Fair and Accurate Machine Learning for Criminal Recidivism Prediction

Objectives: We study interpretable recidivism prediction using machine learning (ML) models and analyze performance in terms of prediction ability, sparsity, and fairness. Unlike previous works, this study trains interpretable models that output probabilities rather than binary predictions, and uses quantitative fairness definitions to assess the models. This study also examines whether models can generalize across geographic locations. Methods: We generated black-box and interpretable ML models on two different criminal recidivism datasets from Florida and Kentucky. We compared predictive performance and fairness of these models against two methods that are currently used in the justice system to predict pretrial recidivism: the Arnold PSA and COMPAS. We evaluated predictive performance of all models on predicting six different types of crime over two time spans. Results: Several interpretable ML models can predict recidivism as well as black-box ML models and are more accurate than COMPAS or the Arnold PSA. These models are potentially useful in practice. Similar to the Arnold PSA, some of these interpretable models can be written down as a simple table. Others can be displayed using a set of visualizations. Our geographic analysis indicates that ML models should be trained separately for separate locations and updated over time. We also present a fairness analysis for the interpretable models. Conclusions: Interpretable machine learning models can perform just as well as non-interpretable methods and currently-used risk assessment scales, in terms of both prediction accuracy and fairness. Machine learning models might be more accurate when trained separately for distinct locations and kept up-to-date.

==> tables/additives_parameter.tex <==
\begin{table*}[htp]
\begin{center}
\tabcolsep=0.1cm
\scriptsize
\caption{Hyperparameters for Additive Stumps}
\label{stumpsparameters_test}
\begin{tabular}{|c|p{2.5cm}|p{2cm}|p{2.7cm}|p{2.7cm}|} \hline

    \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Kentucky}} & \multicolumn{2}{c}{\textbf{Broward}} \\ \hline
    \textbf{Models} & \textbf{Two Year} & \textbf{Six Month} & \textbf{Two Year} & \textbf{Six Month} \\ \hline\hline
    
    %%%
    General &  C \(\in\) [1e-3, 2e-3] &  C \(\in\) [1e-3, 1.5e-3] &  C \(\in\) [1e-2, 2e-2\dots 1e-1] &  C \(\in\) [1e-2, 2e-2\dots 1e-1] \\ \hline
    
    %%%
    Violent & C \(\in\) [6e-4, 8e-4, 1e-3] & C \(\in\) [5e-4, 7e-4] & C \(\in\) [1e-2, 2e-2 \dots 7e-2] & C \(\in\) [1e-2, 2e-2 \dots 7e-2] \\ \hline
    
    %%%
    Drug & C \(\in\) [1e-3, 2e-3, 2.5e-3] & C \(\in\) [1e-3, 2e-3] & C \(\in\) [1e-2, 2e-2 \dots 9e-2] & C \(\in\) [1e-2, 2e-2 \dots 6e-2] \\ \hline

    %%%
    Property & C \(\in\) [1e-3, 1.5e-3] & C \(\in\) [1e-3, 1.5e-3] & C \(\in\) [1e-2, 2e-2 \dots 8e-2] & C \(\in\) [1e-2, 2e-2 \dots 6e-2] \\ \hline

    %%%
    Felony & C \(\in\) [1e-3, 1.5e-3] & C \(\in\) [5e-4, 8e-4] & C \(\in\) [1e-2, 2e-2 \dots 8e-2] & C \(\in\) [1e-2, 2e-2 \dots 8e-2] \\ \hline

    %%%
    Misdemeanor & C \(\in\) [1e-3, 1.5e-3] & C \(\in\) [5e-4, 1e-3] & C \(\in\) [1e-2, 2e-2 \dots 7e-2] & C \(\in\) [1e-2, 2e-2 \dots 7e-2] \\ \hline
    
    \multicolumn{5}{l}{All the models use "balanced" for the class\_weight, "liblinear" for the solver, and $\ell_1$ for the penalty.}
\end{tabular}
\end{center}
\end{table*}


==> tables/models_packages.tex <==
\begin{table}[H]
\begin{center}
\scriptsize
\caption{Models \& Packages}
\begin{tabular}{|c|c|c|} \hline
    \textbf{Models} & \textbf{Acronym} &\textbf{Python Package} \\ \hline\hline
    Logistic Regression ($L_1$) & Logistic(l1) &  \(\texttt{sklearn.linear\_model.LogisticRegression}\) \\ \hline
    Logistic Regression ($L_2$) & Logistic(l2) & \(\texttt{sklearn.linear\_model.LogisticRegression}\) \\ \hline
    LinearSVM & SVM &  \(\texttt{sklearn.svm.LinearSVC}\) \\ \hline
    CART & CART &\(\texttt{sklearn.tree.DecisionTreeClassifier}\) \\ \hline
    Random Forest & RF & \(\texttt{sklearn.ensemble.RandomForestClassifier}\) \\ \hline
    XGBoost & xgb & \(\texttt{xgboost}\) \\ \hline 
    Explainable Boosting Machine & EBM & \(\texttt{interpret}\) \\ \hline
    Additive Stumps & Stumps & \(\texttt{sklearn.linear\_model.LogisticRegression}\) \\ \hline
\end{tabular}
\end{center}
\end{table}
